Visually Indicated Sounds

Objects make distinctive sounds when they are hit or scratched. These sounds reveal aspects of an object's material properties, as well as the actions that produced them. In this paper, we propose the task of predicting what sound an object makes when struck as a way of studying physical interactions within a visual scene. We present an algorithm that synthesizes sound from silent videos of people hitting and scratching objects with a drumstick. This algorithm uses a recurrent neural network to predict sound features from videos and then produces a waveform from these features with an example-based synthesis procedure. We show that the sounds predicted by our model are realistic enough to fool participants in a "real or fake" psychophysical experiment, and that they convey significant information about material properties and physical interactions.

==> fig-confusion.tex <==

%% \begin{figure*}
%%  \centering
%%  % \includegraphics[width=1.0\hsize]{figs/confusion_mats.pdf}
%%  %\includegraphics[width=1.0\hsize]{figs/confusion-mats2.pdf}
%%  %\includegraphics[width=.5\hsize]{figs/confusion-mats2.pdf}
%%  % \includegraphics[width=\hsize]{figs/confusion-mats2.pdf}
%%  \subfloat[Material class confusions]{\includegraphics[width=0.68\linewidth]{figs/confusion-mats2.pdf}}
%%  % \subfloat[Nearest-neighbor accuracy.]{\includegraphics[width=0.23\linewidth]{figs/nn-acc.pdf}}
%%  \subfloat[Nearest-neighbor accuracy.]{\includegraphics[width=0.23\linewidth]{figs/nn-acc.pdf}}
%%  \vspace{-3mm}
%%   \caption{\small \rt{(a)} Material class confusions using a nearest-neighbor
%%     classifier over ground truth sound features (left) or predicted
%%     sound features (\rt{middle}). Each row shows, for the specified class,
%%     the distribution labels among the nearest-neighbors to sounds of
%%     that class. \rt{As a bound on performance, we also show
%%       visual recognition results, in which we train an SVM to directly
%%       predict the material label using {\em fc7} features (\rt{right}). Overall and
%%       class-weighted accuracy are 39.35\% and 25.37\%, respectively.
%%       (b) To quantify the similarity between images, we also measure the
%%       accuracy of a nearest-neighbor matching with {\em fc7} features.}}
%%   \vspace{-1.5mm}
%%  \label{fig:confusion_mats}
%% \end{figure*}



%% \begin{figure}
%%   %\includegraphics[width=0.7\linewidth]{figs/confusion.pdf}
%%   \includegraphics[width=\linewidth]{figs/pred-conf.pdf} 
%%  \vspace{-3mm}
%%   \caption{\small \rt{(a)} Material class confusions using a nearest-neighbor
%%     classifier over ground truth sound features (left) or predicted
%%     sound features (\rt{middle}). Each row shows, for the specified class,
%%     the distribution labels among the nearest-neighbors to sounds of
%%     that class. \rt{As a bound on performance, we also show
%%       visual recognition results, in which we train an SVM to directly
%%       predict the material label using {\em fc7} features (\rt{right}). Overall and
%%       class-weighted accuracy are 39.35\% and 25.37\%, respectively.
%%       (b) To quantify the similarity between images, we also measure the
%%       accuracy of a nearest-neighbor matching with {\em fc7} features.}}
%%   \vspace{-1.5mm}
%%  \label{fig:confusion_mats}
%% \end{figure}
 

